Neural Convolutional Surfaces

This work is concerned with a representation of shapes that disentangles fine, local and possibly repeating geometry, from global, coarse structures. Achieving such disentanglement leads to two unrelated advantages: i) a significant compression in the number of parameters required to represent a given geometry; ii) the ability to manipulate either global geometry, or local details, without harming the other. At the core of our approach lies a novel pipeline and neural architecture, which are optimized to represent one specific atlas, representing one 3D surface. Our pipeline and architecture are designed so that disentanglement of global geometry from local details is accomplished through optimization, in a completely unsupervised manner. We show that this approach achieves better neural shape compression than the state of the art, as well as enabling manipulation and transfer of shape details. Project page at http://geometry.cs.ucl.ac.uk/projects/2022/cnnmaps/ .

==> figures/parametrization.tex <==



\begin{figure}[t]
    \centering
    \begin{tabular}{cc}
        \includegraphics[width=0.48\columnwidth]{pictures/dragon_scales} & 
        \includegraphics[width=0.48\columnwidth]{pictures/dragon_uv_layout} \\
    \end{tabular}
    
    \caption{Parametrization distortion: \label{fig:parametrization}
        this kind of 2D domain is affected by rotation and scale differences, even for similar part of the geometry. The green and orange scale are virtually the same but their 2D counterpart is very different. \luca{this picture might not be included in the final paper, better a small picture beside text?} }
    
\end{figure}



==> figures/pipeline.tex <==

\begin{figure*}[t]
\centering

\includegraphics[width=2\columnwidth,height=4cm]{example-image}

\caption{\textbf{Pipeline image:} TODO}
\label{fig:pipeline}


\end{figure*}


==> includes/old_text.tex <==
Our representation is based on Neural Surface Maps\cite{morreale2021neural}. Figure \ref{fig:architecture} depicts our architecture. A Neural Convolutional Surface $\phi$ consists of two modules: a coarse and a fine network. The coarse network maps 2D coordinates to 3D points $\vertex$. The fine networks displaces the generated coarse vertex to accurately reconstruct the shape. 

%Hence, Neural Convolutional Surface maps 2D point to a point on the surface.
%We supervise it with the ground truth geometry. Due to its limited capacity, the network cannot reconstruct accurately the geometry. 

%Similarly to \cite{morreale2021neural}, we parametrize the shape to a unit cirlce using SLIM\cite{rabinovich2017scalable} and overfit to this $\Real^3 \to \Real^2$ map.

We define the coarse network as shallow MLP. This network is tasked to reconstruct a rough shape, and by doing so it factors out the location information from the representation used by the fine network.


The fine map upsamples a learnable latent code $\latent \in \mathcal{R}^{CxHxW}$ with a CNN to an high resolution feature grid $\gridfeats$. These features are interpolated into a single vector, $\interpfeats$, for each input UV point. Then, a shallow MLP maps $\interpfeats$ to a displacement vector $\displacement$ in a canonical reference frame. We map $\displacement$ onto the coarse reconstruction by analytically computing a Local Reference Frames (LRFs) for each corresponding vertex. Finally, we displace each vertex to generate the fine reconstruction. 


Intuitively, this coarse-fine separation enables weight sharing for similar geometric details. While the coarse map defines a reference global position $\vertex$. The fine map must add geometric texture to it, namely displacing it by $\displacement$. Projecting $\displacement$ on $\vertex$ with the LRF we factor out any global information from $\displacement$, hence the CNN can effectively encode similarly akin geometric details.

% For examples, details such as dragon scales are more likely to activate the same kernels in the convolutional backbone. This concept is similar to the self-similarity assumption from \cite{hanocka2020point2mesh}. 
% should make an example?

Next, we discuss the challenges stemming from the combination of parametrization and convolution.

\subsection{Convolution}

The proposed method indirectly performs convolution on the parametrization domain. This domain is heavily affected by distortion and rotation. Namely, similar parts of the geometry may have different orientations and scales. We address these problems by splitting the surface into small overlapping patches. Each patch $\patch_i$ is independently parametrized, and have a latent code $\latent_i$ associated with it. 


Patches are created from a given shape by random sampling. We select a vertex at random, and extract the subset of mesh with geodesic distance less than 0.04 from it. We parametrize this patch with SLIM\cite{rabinovich2017scalable}, and flag all the vertex in it as selected with a probability of 0.5, hence increasing the overlap between patches. We repeat this process until the whole mesh has been covered, selecting each time an unselected vertex.


Intuitively performing convolution over small patches is comparable to edge detection in images. Each patch extracted from a larger image, \eg face, focuses on a small detail, \eg eye. Since the network is tasked to reconstruct only small patches, it cannot learn to associate meaning to it. On the other hand, it learns to reuse patterns, \ie, edges, present in each patch. In our framework the image is our shape, while the edges are relative displacements making up the geometric texture of the shape.





%\input{figures/parametrization}
\input{figures/pipeline}

In the following we describe the overfitting procedure.
\subsection{Overfitting}

Following \cite{morreale2021neural}, we pre-compute a ground truth map $f:\Real^3 \rightarrow \Real^2$ from the original mesh to a unit circle using SLIM\cite{rabinovich2017scalable}. For each extracted patch, we compute a similar parametrization independently. We store the map between the global parametrization and each local parametrization. In this way we obtain a global to local map.


We use the global parametrization as input to the coarse network and task the network to reconstruct the complete geometry:
\begin{equation} \eqlabel{coarse_loss}
    \mathcal{L}_{coarse} = \int || \phi_{coarse} - f^{-1} || .
\end{equation}
Due to its limited capacity $\phi_{coarse}$ cannot accurately reconstruct the shape. 


We input the local parametrization to the fine network, and predict a displacement vector applied to the corresponding vector on the geometry. We supervise the fine network with the local patch map $f_i$:
\begin{equation} \eqlabel{fine_loss}
    \mathcal{L}_{fine} = \int || \phi - f_i^{-1} || .
\end{equation}


We jointly train both network as follows:
\begin{equation} \eqlabel{train_loss}
    \mathcal{L} = \lambda \mathcal{L}_{coarse} + (1 - \lambda) \mathcal{L}_{fine} ,
\end{equation}
where $\lambda$ is used to transition between the two networks.

\subsection{Joint training}
We train the coarse and fine networks jointly. Since the coarse network implicitly define the LRF by the fine, we warm-up the coarse network, training it for 300K iterations. To do so we set $\lambda=1$ and the step size for the network to $lr_{coarse}=1.0e-4$, while the step size for the fine network is set to $lr_{fine}=0$.

After the warm-up stage we reduce $\lambda$ to 0 over 100K iterations, following cosine annealing \cite{loshchilov2016sgdr}. In parallel, we reduce $lr_{coarse}$ with the same strategy, and increase $lr_{fine}$ up to $1.0e-4$ following $lr_{fine}=1.0e-4 - lr_{coarse}$. After this stage, to allow the coarse network to change we set $lr_{coarse}=1.0e-6$.




\subsection{Shape reconstruction}
To reconstruct the target shape at inference time we assemble each patch weighting corresponding points based on their distance to the origin in their local parametrization. Where points at the origin have weight 1 and at the boundary have weight 0. We set uniform weights to all points in the coarse geometry which belong to only boundary points, hence avoiding artifacts in the reconstruction.


\subsection{minor info}

\begin{itemize}
    \item there is an upsampling layer before each convolution
    \item the convolution is residual (skip connection) to improve reconstruction quality
    \item the size of the coarse mlp depends on the complexity of the final geometry 
    \item the coarse mlp has softplus
    \item the cnn and fine mlp has relu
    \item the latent code has the largest amount of parameters
\end{itemize}


% Then, we overfit a Convolutional Surface Map overfits by jointly supervising the entire architecture and the coarse map:
% \begin{equation} \eqlabel{train_loss}
%     \mathcal{L} = \int|| \phi - f^{-1} || + \lambda \mathcal{L}_{coarse}
% \end{equation}




% \luca{We cannot replace a coarse MLP (global uv $\to$ global coarse) with a set of coarse MLP (local uv $\to$ local coarse) because the local coarse won't be consistent with each other. In particular, LRFs of a vertex $\vertex$ can be different for each patch. This results in different predictions of the Fine MLP (eg different in magnitude) nullifying the reuse. \\ The counter-option is to interpolate each $\vertex$ every time we want to obtaine the LRF. }



% \subsection{Shapes collection}



% \subsection{Interpretability}

% \luca{Discuss collection}



% In the following we describe the overfitting procedure.
% \subsection{Overfitting}

% Following \cite{morreale2021neural}, we overfit the $f^{-1}:\Real^2 \rightarrow \Real^3$. We supervise the entire architecture, as well as the coarse predictor with the ground truth geometry:
% \begin{equation} \eqlabel{train_loss}
%     \mathcal{L} = \int|| \phi - f^{-1} || + \int || \phi_{coarse} - f^{-1} ||
% \end{equation}

% Notice, the coarse predictor $\phi_{coarse}$ has limited capacity, thus it cannot represet accurately the map.


% \subsection{Editing}

% The main goal of this work is to propose an editable and interpretable surface representation. Seminal works, like \cite{bau2020rewriting,bau2018gan}, edit StyleGan images manipulating kernels activations. Given  a layer in the network, the authors first estimate a firing threshold for each neuron in the layer based on statistical information. Hence, a neuron fires, at a specific pixel location, if its activation value is higher than the threshold. Then the authors, estimate the IoU, intersection over union, between the firing neurons and a semantic map of the given concept, e.g., trees. Neurons with an IoU > ? are reacting to the semantic concept.

% Manipulating the activation at firing locations, for example setting it to 0, changes the semantic information conveyed, thus the generated image. For example, authors replace towers ceilings with trees by setting neuron activations associated to towers to the average tree activation value.

% \textbf{This manipulation strategy is very effective, and capable of producing very compelling results. However, since the convolutional network in our map is also responsible for the 3D location we cannot apply the same strategy naively. Indeed, by manipulating features as described, we might perform a global editing, i.e., drastically change the XYZ of points, rather than a local one, i.e., small change of the XYZ coordinates.}

% This can be true even with Neural Subdivision: one feature might encode X, hence setting it to 0 might drastically change the predicted point.

% Big assumption, values can only be positive. This is true in case the network has only RELU. Not in our case since the code can assume any value and we just add to it.

% The solution is to use a Residual Network with RELU activation after every residual. It is not optimal, the performances might decrease because we limit the domain to half space. Hence forcing the network to be linear.

% Should make a single script that modify or edit a region (start specialized: for a given model, then change) the regions are given from a segmentation map

% Editing regions with different distortion (scaling) will respond differently in the same layer.

% The solution can be to edit those region at different layers.

% Remember there is a component in the feature that is associated with the distortion.

% In particular, authors identify neurons responsible for a semantic concept, and manipulate their activation. (should discuss this in more details)

% Following this strategy, we manipulate the convolutional component in our representation to edit the 3D geometry. We perform 3 types of editing:

% - geometry removal
% - geometry cloning
% - geometry enhancement

% \paragraph{Geometry Removal}

% We remove a region $\mathcal{R}$ of the 3D geometry manipulating the activations of the CNN. First, we identify which neurons fire for $\mathcal{R}$ following [2,3,4], using $\mathcal{R}$ as semantic map. Then, in each layer we replace the activations of such neuron with 0. Performing this operation over the entire network ensures the semantic concept is not generated. \luca{figure help here}


% Performing such analysis on the final features do not allow us to identify which feature encodes the geometry. For example, given a feature vector of size 16, the geometry can be encoded around the mean of the first vector element. Following the strategy above, we select a feature only if its activation are close to the statistical maximum value of such feature. Hence, if it is encoded around the mean, we would not manipulate such feature. \luca{review this sentence}


%%%% end method


==> tables/reconstruction.tex <==


\begin{table*}[t]
    \centering
    \caption{Reconstruction quality and compression comparison:
        \label{tab:reconstruction} we compare with state of art method and classic mesh. Our method performs ... wrt the baselines in terms of Euclidean distance (ED) and disk space occupied (MB).}
    
    \begin{tabular}{lc|c|c|c|c|c|c}

        & & Mesh & Mesh zip & NGLOD \cite{takikawa2021neural} & ACORN \cite{martel2021acorn} & NGLOD \cite{takikawa2021nglod} & Ours \\
        \hline
        \multirow{2}{*}{Lucy} & CD & & & & & & \\
                              & MB & & & & & & \\
        \hline
        \multirow{2}{*}{Bimba} & CD & 0.0 & 0.0 & 6.092e-6 & & & 0.646e-06 \\
                               & MB &     &     & 36.8     & & & 0.520 \\
        \hline
        \multirow{2}{*}{Asian Dragon} & ED & & & & & & \\
                                & MB & & & & & & \\
        \hline
        \multirow{2}{*}{Armadillo} & ED & 0.0 & 0.0 & & & & 2.72e-06 \\
                                   & MB & 8.2 & 5.5 & & & & 0.7 \\
        \hline
        \multirow{2}{*}{Ramesses} & ED & & & & & & \\
                                  & MB & & & & & & \\
        \hline
        \multirow{2}{*}{Dragon Warrior} & ED & & & & & & \\
                                        & MB & & & & & & \\
        \hline
        \multirow{2}{*}{Budda} & ED & & & & & & \\
                               & MB & & & & & & \\
        \hline
        
    \end{tabular}
\end{table*}



==> tables/shape_size.tex <==

\begin{table}[h!]
    \centering
    \caption{\label{tab:shape_size}Description of the models used for evaluation.}
    
    \begin{tabular}{r|r|r}
         & \# Vertices & \# Faces \\
         \hline
         \hline
         Armadillo & 172K & 346K \\
         Bimba & 50K & 100K \\
         Ankylosaurus & 26K & 51K \\
         Lucy & 877K & 1753K \\
         Dragon & 451K & 902K \\
    \end{tabular}
    
\end{table}

